Quantization of the Zigzag Model

The zigzag model is a relativistic integrable $N$-body system describing the leading high-energy semiclassical dynamics on the worldsheet of long confining strings in massive adjoint two-dimensional QCD. We discuss quantization of this model. We demonstrate that to achieve a consistent quantization of the model it is necessary to account for the non-trivial geometry of phase space. The resulting Poincar\'e invariant integrable quantum theory is a close cousin of $T\bar{T}$ deformed models.

==> On quantizations of the zigzag model/QM.tex <==
1) Hilbert spaces, probability, measurement, canonical quantization
2) Time evolution, Hamiltonian, Schrodinger  equation, symmetries in QM
3) Pure and mixed states, entanglement
4) Coordinate and momentum representations, uncertainty principle, wave behavior
5) QM potentials in d=1, bound states, reflection and transmission coefficients, tunneling
6) Harmonic oscillator, displaced ground state, coherent states
7) Path Integral, propagators, solving harmonic oscillator with path integral
8) WKB approximation, Bohr-Sommerfeld
9) Rotation group, orbital and spin angular momentum, spherical harmonics
10) Combining angular momentum, Clebsch-Gordon coefficients
11) Schrodinger equation in 3D, hydrogen atom
12) Identical particles, bosons and fermions, periodic table
13) Time-independent perturbation theory, Zeeman and Stark effects
14) Variational method
15) Time-dependent perturbation theory, sudden and adiabatic approximations, Fermi's golden rule 
16) Interactions with  electromagnetic radiation, Aharonov-Bohm effect, absorption and emission of radiation, Landau levels
17) Scattering theory,  Lippman-Schwinger, scattering amplitudes
18) Born approximation
19) Phase shifts and partial waves, scattering cross-section
20) Unitarity and optical theorem 
21) Time delay,  resonances and bound states
20) Eikonal (WKB) approximation for scattering
21) Coulomb scattering

==> QM.tex <==
1) Hilbert spaces, probability, measurement, canonical quantization
2) Time evolution, Hamiltonian, Schrodinger  equation, symmetries in QM
3) Pure and mixed states, entanglement
4) Coordinate and momentum representations, uncertainty principle, wave behavior
5) QM potentials in d=1, bound states, reflection and transmission coefficients, tunneling
6) Harmonic oscillator, displaced ground state, coherent states
7) Path Integral, propagators, solving harmonic oscillator with path integral
8) WKB approximation, Bohr-Sommerfeld
9) Rotation group, orbital and spin angular momentum, spherical harmonics
10) Combining angular momentum, Clebsch-Gordon coefficients
11) Schrodinger equation in 3D, hydrogen atom
12) Identical particles, bosons and fermions, periodic table
13) Time-independent perturbation theory, Zeeman and Stark effects
14) Variational method
15) Time-dependent perturbation theory, sudden and adiabatic approximations, Fermi's golden rule 
16) Interactions with  electromagnetic radiation, Aharonov-Bohm effect, absorption and emission of radiation, Landau levels
17) Scattering theory,  Lippman-Schwinger, scattering amplitudes
18) Born approximation
19) Phase shifts and partial waves, scattering cross-section
20) Unitarity and optical theorem 
21) Time delay,  resonances and bound states
20) Eikonal (WKB) approximation for scattering
21) Coulomb scattering
